A Collisional-Energy-Cascade Model for Nonthermal Velocity Distributions of Neutral Atoms in Plasmas

Nonthermal velocity distributions with much greater tails than the Maxwellian have been observed for radical atoms in plasmas for a long time. Historically, such velocity distributions have been modeled by a two-temperature Maxwell distribution. In this paper, I propose a model based on collisional energy cascade, which has been studied in the field of granular materials. In the collisional energy cascade, a particle ensemble undergoes energy input at the high-energy region, entropy production by elastic collisions among particles, and energy dissipation. For radical atoms, energy input may be caused by the Franck-Condon energy of molecular dissociation or charge-exchange collision with hot ions, and the input energy is eventually dissipated by collisions with the walls. I show that the steady-state velocity distribution in the collisional energy cascade is approximated by the generalized Mittag-Leffler distribution, which is a one-parameter extension of the Maxwell distribution. This parameter indicates the degree of the nonthermality and is related to the relative importance of energy dissipation over entropy production. This model is compared with a direct molecular dynamics simulation for a simplified gaseous system with energy input and dissipative wall collisions, as well as some experimentally observed velocity distributions of light radicals in plasmas.

==> latexmkrc <==
#!/usr/bin/perl
$latex         = 'pdflatex %O -src-specials -shell-escape -interaction=nonstopmode -synctex=1 main';
$bibtex        = 'pbibtex %O %B';
$dvipdf        = 'dvipdfmx %O -o %D main_supplemental';
$pdf_mode      = 3; # use dvipdfmx

# Use SumatraPDF and atom inverse search
# $pdf_previewer = '"C:\Program Files\SumatraPDF\SumatraPDF.exe" -reuse-instance -inverse-search "\"%USERPROFILE%\AppData\Local\atom\bin\atom.cmd\" \"%f:%l\"" %O %S';

# if you do not need to preview in -pvc option (preview document and countinuously update mode)
# $pdf_previewer = 'exit';

